EVAN: Evolutional Video Streaming Adaptation via Neural Representation

Adaptive bitrate (ABR) using conventional codecs cannot further modify the bitrate once a decision has been made, exhibiting limited adaptation capability. This may result in either overly conservative or overly aggressive bitrate selection, which could cause either inefficient utilization of the network bandwidth or frequent re-buffering, respectively. Neural representation for video (NeRV), which embeds the video content into neural network weights, allows video reconstruction with incomplete models. Specifically, the recovery of one frame can be achieved without relying on the decoding of adjacent frames. NeRV has the potential to provide high video reconstruction quality and, more importantly, pave the way for developing more flexible ABR strategies for video transmission. In this work, a new framework, named Evolutional Video streaming Adaptation via Neural representation (EVAN), which can adaptively transmit NeRV models based on soft actor-critic (SAC) reinforcement learning, is proposed. EVAN is trained with a more exploitative strategy and utilizes progressive playback to avoid re-buffering. Experiments showed that EVAN can outperform existing ABRs with 50% reduction in re-buffering and achieve nearly 20% .

==> store.tex <==
\paragraph{Soft Actor-Critic ABR}
A variety of different RL algorithms have been applied to solve complex adaptive bitrate problems. In our design, we chose to use soft actor-critic (SAC) since, to our best knowledge, it is the state-of-the-art and has been successfully proven to better trade-off exploration and exploitation during the training of an agent. Due to the limited exploration of the A3C policy, sometimes, in order to eliminate rebuffering completely, relatively conservative bitrate selections are made. This strategy does not benefit the progressive playback of NeRV. In EVAN, we aim to select higher bitrates whenever possible, even if there is some degree of rebuffering, as it can be mitigated through progressive playback. SAC approximates the policy towards the Q-function, thus avoiding getting stuck in local optima and encouraging exploration of other actions. This approach enables higher bitrate decisions, while NeRV's progressive playback can reduce rebuffering if the action is too aggressive. 
Fig. \ref{fig:1} shows the SAC architecture, which includes an actor network for decision probability distribution and two Q-networks for state-action value estimation. Weights between Q-networks are periodically alternated to prevent overestimation of Q-values. Each Q-network consist of one evaluation network (Q-evaluation) and the target network (Q-target) to optimize Q-evaluation, which are used to estimate the current and target Q values in Bellman equation. 
The aim of A3C is to maximize the cumulative rewards, with exploitation only taking place during the gradient decent phase. In contrast, SAC considers jointly maximize the cumulative rewards and the entropy in the training goal. For each policy iteration, agents choose the optimal policy that maximizes the weighted sum of expected cumulative reward and entropy:
\begin{equation}
    \pi^* = \underset{\pi}{\rm \text{argmax}}
    \; \mathbb{E}_{a_t \sim \pi} r(s_t,a_t) + \beta \mathcal{H}(\pi(\dot|s_t))
\end{equation}
The value function of SAC can be determined by the Bellman equation as:
\begin{equation}
    \begin{aligned}
        & \underset{\pi}{\rm \text{max}} 
        & & V(s_t) = \mathbb{E}_{a_t \sim \pi} Q(s_t,a_t)-\beta log(\pi(a_t|s_t)) \\
    \end{aligned}
    \label{bellman}
\end{equation}
It is evident that when entropy is included in the objective, the optimization goal is equivalent to minize the KL divergence between the policy probability and the "Q-shaped" probability distribution. This is in line with the SAC design idea as we have discussed at the start of this section. Details of the SAC network are explained below:\\
\begin{itemize}
    \item Inputs: At the client side, after each model at $t$ is downloaded, the agent takes state input $s_t$ as $s_t = (\boldsymbol{x_t},\boldsymbol{\tau_t},\boldsymbol{n_t},B_t, C_t, l_m)$, where $\boldsymbol{x_t}$ is the vector stores past model download throughput, $\boldsymbol{\tau_t}$ stores past model download time, $\boldsymbol{n_t}$ stores the available model sizes for next chunk, $B_t$ is current buffer size, $C_t$ is last chunk's bitrate and $l_m$ is the number of unplayed video chunks.
    \item Actor network: The aim of the policy network is to minimize the KL divergence of the policy distribution and the "Q shaped" probability distribution. We can write the expression of actor network $J_\pi(\phi)$ loss as:
    \begin{small}
    \begin{equation}
        \begin{aligned} J_\pi(\phi) & =D_{\mathrm{KL}}\left(\pi_\phi\left(. \mid s_t\right) \| \exp \left(\frac{1}{\beta} Q_\theta\left(s_t, .\right)-\log Z\left(s_t\right)\right)\right) \\ & =\mathbb{E}_{a_t \sim \pi_\phi}\left[\log \left(\frac{\pi_\phi\left(a_t \mid s_t\right)}{\exp \left(\frac{1}{\beta} Q_\theta\left(s_t, a_t\right)-\log Z\left(s_t\right)\right)}\right)\right] \\ & \end{aligned}
    \end{equation}
    \end{small}
$\pi_\phi$ is the actor policy, $Q_{\theta}$ is Q-value estimated from Q network. $\beta$ is the weight of entropy, which is called entropy temperature and $\log Z(s_t)$ is the log partition function. To ensure the whole process is differentiable, actions are sampled using reparameterization tricks. Since $\log Z(s_t)$ does not affect the calculation of actor network gradient, we can update the actor network weights $\phi$ as:
\begin{small}
\begin{equation}
    \phi \leftarrow \phi + \alpha \nabla_{\phi}(\mathbb{E}_{a_t \sim \pi_\phi}\left[\log \pi_\phi\left(a_t \mid s_t\right)-\frac{1}{\beta} Q_\theta\left(s_t, a_t\right)\right])
    \label{gradient}
\end{equation}
\end{small}
\item Q network: 
The Q network is used to approximate the state-action value generated during the agent-environment interaction. Q network is trained to maximize the advantage function $A(a_t, s_t)$:
\begin{equation}
    A(a_t, s_t) = Q\left(s_t, a_t\right)-(r\left(s_t, a_t\right)+\gamma V\left(s_{t+1}\right))
\end{equation}
As we have mentioned, Q-evaluation network $Q_{\theta}$ here is trained to estimate current Q value $Q\left(s_t, a_t\right)$ while Q-target network $Q_{\bar{\theta}}$ is trained to estimate the target Q value. By replacing $Q(s_t, a_t)$ in Eq. \ref{bellman} with the esimated Q target, we obtained the state value $V(s_t)$ to calculate the advantage. The training loss for the Q network is:
\begin{small}
\begin{equation}
\begin{aligned}
J_Q(\theta) & = \mathbb{E}_{\pi_{\phi}}\left[\frac{1}{2}A(a_t, s_t)^2\right]  = \mathbb{E}_{\pi_\phi}\left[\frac{1}{2}\left(Q_\theta\left(s_t, a_t\right) -\left(r\left(s_t, a_t\right) \\ & + \right. \right. \left. \left. \gamma\left(Q_{\bar{\theta}}\left(s_{t+1}, a_{t+1}\right) 
-\beta \log \left(\pi_\phi\left(a_{t+1} \mid s_{t+1}\right)\right)\right)\right)\right)^2\right]
\end{aligned}
\end{equation}
\end{small}
\item Entropy finetune: In our design, we dynamically adjust the entropy weight by gradient descent. Specifically, we start by setting an entropy threshold, denoted as $\mathcal{H}_0$. we follow the suggestion of [] to set $\mathcal{H}_0$ as $\mathcal{H}_0 = 0.98(\log (\text{dim}(a_t))$. Then, in each epoch, we employ gradient descent to adjust the weight so that the entropy approaches the target $\mathcal{H}_0$:
\begin{equation}
    \beta \leftarrow \beta - \alpha(\mathcal{H}(\pi(\dot|s_t)) - \mathcal{H}_0)
\end{equation}
This enables a more reasonable alteration of the effect of entropy and reward during the RL agent's training.
\end{itemize}



 We train a selection of NeRV models using video representations from \cite{waterloo}. PSNRs of the reconstructed videos are recorded in relation to different NeRV sizes, which is utilized for NeRV bitrate mapping. NeRV models are built with different hyperparameters to ensure their sizes are compatible with the video chunk sizes. NeRV takes frame index as input and passes it through the MLP network to generate a feature map. The feature map is then upscaled in size through multiple NeRV blocks that are connected together, resulting in the final output frame. MLP feature map is set with the length-and-width ratio of the video, which is relatively fixed. Therefore, we need to adjust the upscale vector to generate videos with different resolutions. For example, for a 1080p video, the MLP feature map is (9,16), in order to generate the frame size with 3840*1920, we can set the upscale vector as [5, 3, 2, 2, 2]. It is far from enough to only adjust the upscale vector since a higher video resolution usually requires a larger hidden space to represent the video's finer grained features. Therefore, we further modify the number of channels and the size of the hidden dimension in order to enhance the video quality. As Fig. \ref{a} shows, the PSNRs of the reconstructed videos demonstrate that NeRV has a clear superiority over traditional H.264 encoding in the low BPP range. This allows for higher video quality transmission with limited bandwidth. We measure the video-reconstruction quality for different downloading ratios by pruning the models and measuring the PSNRs of the reconstructed videos. The results suggest that most NeRV models can achieve a satisfactory playback quality with more than 40\% weights pruned. Fig. \ref{b} shows the reconstructed frames from the "owl" chunk. The quality of the reconstructed frames is still quite good and visually pleasing within a certain pruning range.

